Internal and external pressures on language emergence: least effort, object constancy and frequency

In previous work, artificial agents were shown to achieve almost perfect accuracy in referential games where they have to communicate to identify images. Nevertheless, the resulting communication protocols rarely display salient features of natural languages, such as compositionality. In this paper, we propose some realistic sources of pressure on communication that avert this outcome. More specifically, we formalise the principle of least effort through an auxiliary objective. Moreover, we explore several game variants, inspired by the principle of object constancy, in which we alter the frequency, position, and luminosity of the objects in the images. We perform an extensive analysis on their effect through compositionality metrics, diagnostic classifiers, and zero-shot evaluation. Our findings reveal that the proposed sources of pressure result in emerging languages with less redundancy, more focus on high-level conceptual information, and better abilities of generalisation. Overall, our contributions reduce the gap between emergent and natural languages.

==> approach.tex <==
\section{Setup}
\label{sec:approach}

We study language emergence in the context of task-oriented multi-agent games.
In the current section, we present our baseline setup (\S~\ref{sec:game_description}) and the original dataset (\S~\ref{sec:data}).
% As baseline, we use the setup of \citet{havrylov2017emergence} (see Section~\ref{sec:game_description}, with images from the SHAPES dataset introduced by \citet{Andreas_2016} (see Section~\ref{sec:game_description} and Section~\ref{sec:data} below).
% \dieuwke{We then introduce three variants of this setup, that relate to three different \ldots}

\subsection{Game definition}
\label{sec:game_description}
% Sender-Receiver setup
% [less than a column] 
% Here you describe our setup; you should stay as data-agnostic as possible (e.g., not binding the description to a particular dataset, such as SHAPES); you could take inspiration from how Lazaridou or Titov introduce it.

In the game we study, two agents play a referential game. One agent, the Sender, has to describe an image; the other agent, the Receiver, has to pick the correct image out of a line-up of confounders. We follow the setup of \citet{havrylov2017emergence}:
\begin{enumerate}
\item There are $N$ images represented by z-dimensional feature vectors $f_n=\{i_1,...,i_z\}$. A target image $t$ is sampled and shown to the Sender.
\item The Sender generates a message $m$ with a maximum length $L$ that consists of a sequence of words $\{w_i, \dots, w_{\leq L}\}$ from a vocabulary of size $|V|$.
\item The Receiver uses $m$ to identify $t$ in a set of images that contains $k$ distracting images and $t$ in random order.
\end{enumerate}

We implement both the Sender and Receiver agents as LSTM networks. Unless otherwise specified, we follow again the training procedures and error definitions of \citet{havrylov2017emergence}.\footnote{For brevity, we omit them from the full paper, but report them in Appendix~A.}
A scheme of this setup is shown in Figure~\ref{fig:modelDiagram}.

\begin{figure*}
\center
\includegraphics[width=.8\textwidth, trim=0mm 3mm 0mm 2mm, clip]{modelDiagram.png}
\caption{Architecture overview of the Sender and Receiver. The visual module shows the CNN architecture used for extracting features from the input.}
\label{fig:modelDiagram}
\end{figure*}

\subsection{Data}\label{sec:data}

We use images from a modified version of the SHAPES dataset \citep{Andreas_2016}. This dataset consists of a series of 30 x 30 pixel images. Each image contains exactly one 2D object, which is characterised by a shape (circle, square, triangle), a colour (red, green, blue), and a size (small, big). 
The objects are positioned in a logical grid of three rows and three columns. In the baseline setting, 
we sample both images and distractors uniformly from the images in this space. In the next section, we introduce three alternative versions of the game, in which images are selected following more naturalistic procedures.\footnote{While we work on synthetic data, the same expedients can be easily applied to natural datasets like COCO \citep{lin2014microsoft}.}



==> related_work.tex <==
\section{Motivation}
\label{sec:related_work}
The proposed sources of pressure on emergent languages are motivated on the basis of general principles of human communication and perception. In this section, we outline the principles of least effort, object constancy, and object frequency.

\subsection{Least Effort}
\label{ssec:leasteffort}
While human speakers try to maximise the distinctiveness of the information conveyed, they also minimise the effort involved. A version of this principle was originally formulated by \citet[p. 29]{zipf1935psycho} -- who pointed out the correlation between word frequency rank and word length -- and was later generalised to every reduction of linguistic expressions by \citet{haiman1983iconic} under the name `Principle of Economy.' This principle is also reminiscent of the  maxim of quantity in pragmatics \citep{grice1975logic,levinson2000presumptive}, which requires to give no more information than needed. 

As this principle is a key factor in explaining the variation of natural languages \citep{haiman1983iconic}, it posits a realistic constraint on language emergence. Moreover, our operationalisation of the principle allows the model to determine automatically the maximum length of sequences and the number of symbols in its vocabulary. In doing so, the complexity of the emergent language is gauged according to the data and task at hand. This has the methodological advantage of not requiring to preset these hyper-parameters arbitrarily or performing grid search on task accuracy (which rarely corresponds to natural language properties).

\subsection{Subjective Constancy}
\label{ssec:objconst}

Reality as it is immediately sensed is shapeless and ever-changing. However, animals evolved to various degrees the ability to perceive a reality of objects, namely constant and discrete entities lying behind the tangle of sensation \citep{lorenz1977behind}. 
The same ability is connected with abstraction: over repeated impressions, animals learn to neglect what is contingent (due to the environment or their internal disposition), and group instances of objects with recurring patterns into the same conceptual class \citep{gillam2000perceptual}. 

Object constancy involves several different and independent mechanisms, regarding, among others: i) the \textbf{colour} of the object, under different light conditions \citep{holst1957aktive}; ii) the \textbf{position} of the object, under different perspectives \citep{von1970verhaltensphysiologie}. For instance, bees have to identify flowers by their colour independently from the time of the day (red of dusk or gold of dawn). In our implementation, we manipulate the images in such a way that agents are exposed to the same object with different position or colour. As a consequence, we expect the agents to acquire some sort of constancy mechanisms.
%, to the extent that is beneficial to the task solution. While in animals constancy and abstraction derive from an ontogenetically stable neuro-physiological apparatus, such apparatus is similarly evolved to increase the fitness of the animal's species to the environment phylogenetically.

\subsection{Object Frequency}
\label{ssec:objfreq}
The distribution of objects and features in the real world are highly non-uniform. Agents encounter objects in the environment with different frequencies. Furthermore, the degree of association between features and objects can vary: for instance, berries evoke the colour blue less vividly than the sky. Frequency facilitates the correct classification of object instances \citep{nosofsky1988similarity}. Moreover, \citet{medin1978context} have shown that more frequent stimuli lead to an increasing perceptual differentiation in the region of their features. As a consequence, agents are imprinted with respect to specific features rather than the stimulus as a whole, and stimuli become decomposable into their `building blocks' \citep{schyns1998development}. Recently, \citet{hendrickson2019cross} have also shown how a Zipfian distribution of words and referents can accelerate word meaning acquisition compared to a uniform one.


\iffalse
\subsection{Language emergence in referential games}
Language evolution studies the emergence of language in relation to its function and views it as a result of social interaction \citep{Scott-Phillips2010-SCOLEI}.
Based on the language evolution theory, recent studies have used deep learning to show that communication protocols can emerge out of the necessity of coordinating agents to accomplish a task \cite{cao2018emergent}.
Referential games are often used in language emergence experiments under a reinforcement learning context in which neural agents cooperate to win the game.
Specifically, the Lewis signaling game \citep{Lewis1969-LEWCAP-4} and variations of it have been extensively used in the field.
A sender and a receiver agent interact to play this game.

Many different game setups have been explored.
Early games use symbolic input which is highly structured \citep{mordatch2017emergence, Andreas_2017}.
Later games use raw pixel data as input since it is more realistic \citep{lazaridou2016multiagent, lazaridou2018emergence}.
It has been shown that the inherent structure of the input is retained in the emerged communication protocol, so it is more challenging for visual input to produce a structured language \cite{lazaridou2018emergence}

There has been experimenting with agents that exchange messages consisting of a single token \citep{lazaridou2016multiagent, jorge2016learning} or of a sequence of tokens of a variable length \citep{havrylov2017emergence}.
The latter is preferred as it resembles natural language more closely and therefore can induce similar properties such as composition of words or hierarchical properties \cite{havrylov2017emergence}.

Other variations have also been explored, such as alternating roles between the sender and the receiver \citep{choi2018compositional}, having a community of agents \citep{mordatch2017emergence} or agents with different cooperation policies \citep{cao2018emergent}.

In all these variations, the agents tend to converge to using a language and successfully solve the tasks.
However, communication success does not always imply a correlation between the input space and the agents' internal mappings of the inputs \cite{bouchacourt2018agents}. In fact, it has been found that there must be an environment pressure to encourage the language to exhibit properties that natural language has, such as compositionality \cite{kottur2017natural}. The input and the game complexity highly influence the properties of the emerged language.
\fi

